Learning Causal Representations from General Environments: Identifiability and Intrinsic Ambiguity

We study causal representation learning, the task of recovering high-level latent variables and their causal relationships in the form of a causal graph from low-level observed data (such as text and images), assuming access to observations generated from multiple environments. Prior results on the identifiability of causal representations typically assume access to single-node interventions which is rather unrealistic in practice, since the latent variables are unknown in the first place. In this work, we provide the first identifiability results based on data that stem from general environments. We show that for linear causal models, while the causal graph can be fully recovered, the latent variables are only identified up to the surrounded-node ambiguity (SNA) \citep{varici2023score}. We provide a counterpart of our guarantee, showing that SNA is basically unavoidable in our setting. We also propose an algorithm, \texttt{LiNGCReL} which provably recovers the ground-truth model up to SNA, and we demonstrate its effectiveness via numerical experiments. Finally, we consider general non-parametric causal models and show that the same identification barrier holds when assuming access to groups of soft single-node interventions.

==> Sections/ambiguity.tex <==
In the previous sections, we prove identifiability under $\sim_{\dom}$ for non-parametric causal models with single-node soft interventions, and for linear causal models with general environments. We have also seen in \Cref{example:discount-revisit} that some ambiguities exist when we cannot remove causal relationships between variables.  However, it is still unknown whether $\sim_{\dom}$ is the best we can hope for in general. In this section, we give an affirmative answer to this question by showing that the ambiguity induced by $\sim_{\dom}$, which we refer to as the \textit{surrounded-node ambiguity} (SNA), is inevitable in the setup of this paper.

We first present a result that serves as a good starting point to understand why this is the case. It states that latent representations that are equivalent under $\sim_{\dom}$ are essentially generated from the same causal graph.

\begin{proposition}
\label{prop:sp-linear-same-graph}
    Let $\mM$ be an invertible matrix such that $\mM_{ij}\neq 0 \Rightarrow j\in\overline{\dom}_{\G}(i)$. Suppose that the latent variables $\vz\in\R^d$ are generated from any distributions $p_i\left(\vz_i\mid\vz_{\pa_{\G}(i)}\right), i\in[d]$ with joint density $p(\vz)=\prod_{i=1}^d p_i\left(\vz_i\mid\vz_{\pa_{\G}(i)}\right)$ 
    , then the joint density of $\vv = \mM \vz$ can be written as $q(\vv)=\prod_{i=1}^d q_i\left(\vv_i\mid\vv_{\pa_{\G}(i)}\right)$ for some density functions $q_i, i\in[d]$.
\end{proposition}

%While \Cref{prop:sp-linear-same-graph} implies that SNA cannot be resolved by examining the structure of the causal graph, it is still unclear whether the ambiguity still exists if we make additional assumptions on the causal model and the environments. 

Finally we state the main theorem in this section, which indicates that the identifiability guarantees in \Cref{thm:linear-main-thm,thm:single-node-soft-nonparam} cannot be improved. %The main results of this section are stated below, indicating that the identifiability guarantees in \Cref{thm:linear-main-thm,thm:single-node-soft-nonparam} cannot be improved, even if additional restrictions on the model are imposed.

\begin{theorem}[Counterpart to \Cref{thm:linear-main-thm,thm:single-node-soft-nonparam}, informal version of \Cref{thm:linear-ambiguity,thm:non-param-ambiguity}]
\label{thm:informal-non-param-ambiguity}
    For any linear causal model $(\mH,\G)$ and any set of environments $\mathfrak{E}=\left\{E_k: k\in[K]\right\}$ such that all conditions in \Cref{thm:linear-main-thm} are satisfied, there must exists a candidate solution $(\hat{\mH},\G)$ and a hypothetical data generating process that satisfy the same set of conditions, but
    \begin{equation}
        \notag
        \frac{\partial \vv_i}{\partial \vz_j} \neq 0,\quad \forall j\in\overline{\dom}_{\G}(i).
    \end{equation}
    Moreover, if we additionally assume that the environments are groups of single-node soft interventions, then we can guarantee the existence of $(\hat{\mH},\G)$ and weight matrices which, besides the properties listed above, are also groups of single-node soft interventions.

    Finally, the same result holds for the non-parametric causal model $(\vh,\G)$ under the setting of \Cref{thm:single-node-soft-nonparam}, and assuming standard axioms such as causal minimality (\Cref{asmp:minimality}) and faithfulness (\Cref{asmp:faithfulness}) on the causal graph would not resolve the SNA either. 
\end{theorem}

Formal statement and the proof of \Cref{thm:informal-linear-ambiguity} can be found in \Cref{appsec:ambiguity}. 

